Understanding AR Activism: An Interview Study with Creators of Augmented Reality Experiences for Social Change

The rise of consumer augmented reality (AR) technology has opened up new possibilities for interventions intended to disrupt and subvert cultural conventions. From defacing corporate logos to erecting geofenced digital monuments, more and more people are creating AR experiences for social causes. We sought to understand this new form of activism, including why people use AR for these purposes, opportunities and challenges in using it, and how well it can support activist goals. We conducted semi-structured interviews with twenty people involved in projects that used AR for a social cause across six different countries. We found that AR can overcome physical world limitations of activism to convey immersive, multilayered narratives that aim to reveal invisible histories and perspectives. At the same time, people experienced challenges in creating, maintaining, and distributing their AR experiences to audiences. We discuss open questions and opportunities for creating AR tools and experiences for social change.

==> columns.tex <==
Participant ID	
Creators	
Project Name	
Creator Type	
Source	Social cause	
How are they using AR?	
Why Interviewing ?	
How the project connects to activism and AR?	
Description of the project	link	
start year	
Place-based	
Contact Info	
Contact email	
Platform	
Technology Used	
Have been contacted in the past?	
Responded	
Interviewed	
Fitness to the Project	
Augmented Sense	
Strong Activism	
Strong AR	
Contact First	
Contacted During Internship	
Responded During Internship	
Interviewed During Internship	
Recommended By Interviewee	
Other comments	
